Embodied Active Defense: Leveraging Recurrent Feedback to Counter Adversarial Patches

The vulnerability of deep neural networks to adversarial patches has motivated numerous defense strategies for boosting model robustness. However, the prevailing defenses depend on single observation or pre-established adversary information to counter adversarial patches, often failing to be confronted with unseen or adaptive adversarial attacks and easily exhibiting unsatisfying performance in dynamic 3D environments. Inspired by active human perception and recurrent feedback mechanisms, we develop Embodied Active Defense (EAD), a proactive defensive strategy that actively contextualizes environmental information to address misaligned adversarial patches in 3D real-world settings. To achieve this, EAD develops two central recurrent sub-modules, i.e., a perception module and a policy module, to implement two critical functions of active vision. These models recurrently process a series of beliefs and observations, facilitating progressive refinement of their comprehension of the target object and enabling the development of strategic actions to counter adversarial patches in 3D environments. To optimize learning efficiency, we incorporate a differentiable approximation of environmental dynamics and deploy patches that are agnostic to the adversary strategies. Extensive experiments demonstrate that EAD substantially enhances robustness against a variety of patches within just a few steps through its action policy in safety-critical tasks (e.g., face recognition and object detection), without compromising standard accuracy. Furthermore, due to the attack-agnostic characteristic, EAD facilitates excellent generalization to unseen attacks, diminishing the averaged attack success rate by 95 percent across a range of unseen adversarial attacks.

==> history/rebuttal_md.tex <==
# Reply

## Reviewer iMPU

Thank you for your insightful and detailed review of our submission. Your feedback has been invaluable in enhancing the clarity and solidity of our research. Below are our responses to your queries:

1. **Computational Overhead:** _How does the computational cost of the proposed method compare to the baselines?_

    > We appreciate your query regarding the computational cost of our method compared to the baselines. Our approach does exhibit a higher computational overhead in both the training and testing phases, as indicated in Table 1. Notably, our EAD method demonstrates superior performance, justifying this increased overhead.
    >
    > ? We compare our method with the other passive defense baselines. We can tell from the results that our method achieves a better performance with considerable computational overhead in both the training and test phases. 
    >
    > *Table 1. Computational overhead comparison of different defense methods in face recognition. We report the training and inference time of defense on a NVIDIA GeForce RTX 3090 Ti and an AMD EPYC 7302 16-Core Processor with the training batch size as 64.* 
    >
    > | **Method** | **# Params (M)** | **Description**                    | **Training Epochs** | **Training Time per batch (s)** | **Inference Time per instance (ms)** |
    > | ---------- | ---------------- | ---------------------------------- | ------------------- | ------------------------------- | ------------------------------------ |
    > | JPEG       | -                | non-parametric                     | -                   | -                               | 9.65                                 |
    > | LGS        | -                | non-parametric                     | -                   | -                               | 26.22                                |
    > | SAC        | 44.71            | segmenter                          | 50 + 10             | 0.152 / 4.018                   | 26.43                                |
    > | PZ         | 44.71            | segmenter                          | 50 + 10             | 0.152 / 4.018                   | 11.88                                |
    > | DOA        | 43.63            | adversarial training               | 100                 | 1.73                            | 8.10                                 |
    > | EAD (ours) | 57.30            | policy model and perception  model | 50 + 50             | 0.595 / 1.021                   | 38.38 (4 steps)                      |
    >
    > We have conducted training of the EAD model with the configuration as detailed in Appendix C.4. The initial offline training phase on 2 NVIDIA Tesla A100 GPUs took approximately 4 hours (210 min), Owing to the huge memory consumption of EG3D differential rendering, we resort to train EAD with 8 NVIDIA Tesla A100 in the online training phase, and it lasts about 14 hours (867 min). These details, along with the training curves, are now included in the updated appendix.

2. **Implementation of Adaptive Attack:** _How does the method fare against an adaptive attack targeting the weakest component in the pipeline?_

    >  Following your valuable advice, we have designed three new adaptive attacks to evaluate the robustness of the EAD model. These attacks target the perception model, the policy model, and the entire pipeline, respectively: 1) attack the perception model to disrupt the model belief (perception)according to your advice and the work by Sabour et. al.  2) attack the policy model (policy) to make it ensure zero action (i.e. EAD model stay stills) 3) Luckily, we succeed in attacking the whole pipeline along 4-steps trajectory with gradient-checkpointing technique (overall) which hasn't been used previously. 
    >
    >  *Table 2. Evaluation of adaptive attacks on the EAD Model. Columns with \emph{USP} represent results obtained by optimizing the patch with an expected gradient over the Uniform Superset Policy (USP). And \emph{perception} and \emph{policy} separately represent adaptive attacks against a single sub-module. And \emph{overall} denotes attacking EAD by following the gradients along the overall (4 step) trajectory with gradient checkpointing.* 
    >
    >  |             | **Dodging** |                |            |             | **Impersonation** |                |            |             |
    >  | :---------: | ----------- | :------------: | :--------: | :---------: | :---------------: | :------------: | :--------: | :---------: |
    >  |             | **USP**     | **Perception** | **Policy** | **Overall** |      **USP**      | **Perception** | **Policy** | **Overall** |
    >  | **ASR (%)** | **22.11**   |     10.11      |   16.84    |    15.79    |       8.33        |      1.04      |  **9.38**  |    7.29     |
    >
    >  The results, as shown in the table, highlight that our original adaptive attack with Uniform Superset Policy (USP) is the most effective in dodging attacks. Though faced with diverse adaptive attacks, our method remains effective. The detailed methodologies of these adaptive attacks are now illustrated in the revised appendix.

3. _Theoretical results relating to approximations used in Sec 3.3._

    >  Our method is built upon the theoretical principles of information theory. We acknowledge that there are several approximations in our implementation that warrant further exploration for a comprehensive theoretical analysis.

4. _Enhanced SAC's robustness against dodging attacks compared to regular SAC._

    >  The  SAC first adopts a segmentation model to detect patch areas, followed by a "robust complementation" technique to extend the predicted area into a larger square, masking the predicted padded area. In scenarios like adversarial glasses attacks, the enhanced SAC, trained with adversarial examples, exhibits improved segmentation performance. This results in more significant occlusion in the image, particularly covering critical facial features like eyes and noses (as demonstrated in the qualitative comparison of enhanced SAC and its regular counterparts). Consequently, the Face Recognition (FR) model tends to misidentify the occluded face as a different identity, leading to decreased performance in dodging attacks.

    We hope these responses address your concerns satisfactorily. We are committed to continually improving our work and are grateful for your constructive feedback.

## Reviewer V4oi

First and foremost, I would like to extend my heartfelt gratitude for your thorough and insightful review of our manuscript. Your attention to detail and rigorous assessment have significantly contributed to the enhancement of our paper. We deeply apologize for the typos and other errors in our previous draft. Your meticulousness in identifying these issues has been invaluable, and we have made concerted efforts to rectify these oversights in our revised manuscript.

In response to your comments, we have made the following revisions and additions:

1. Improvement of writing.

    > 1.1	We have included an introduction to the tasks of Impersonation and Dodging in the updated appendix, ensuring clarity and comprehensiveness.
    >
    > 1.2	The environmental setting for object detection is indeed similar to that of face recognition, with the primary distinction being the feasible region of viewpoints. We have added a concise summary in the appendix to clarify this aspect.
    >
    > 1.3	The explanation for the attacks used has been elaborated in the appendix for better understanding.
    >
    > 1.4	The notation of model prediction is now clearly defined in the revised background section.
    >
    > 1.5	We will provide a detailed outline of the codebase, along with a brief guide for its execution, in the near future.
    >
    > We have diligently corrected the typos and flaws, particularly those highlighted in your review. We sincerely apologize for our previous carelessness in writing and have made every effort to minimize such errors in the revised version of our paper.

2. The paper makes a claim that passive adversarial defense approaches are not sufficient for a dynamic environment. This claim should be supported by a passive defense used as a baseline. Also, it would be great to see the extra amount of training resources used to train the active embodied model vs a passive defense approach (for eg Madry's PGD adversarial training). It would also help the readers if some other active defenses would be used as a baseline in order to establish the efficacy of the proposed approach.

    > We acknowledge the need for a baseline comparison with passive defense methods. Our paper includes a comparison with DoA, which can be considered as the patch version of Madry's PGD adversarial training In the meantime, we already use 3D-augmented data (image observed from various viewpoints) to train the passive baseline, which we forgot to claim in our paper previously, we apologize for our mistakes. As shown in the table,  the passive defense baseline with only 2D data is less robust than the ones trained with 3D-augmented data (baseline in the paper). As for other active defenses, they are currently unavailable to the best of our knowledge. 
    >
    > *Table 1. Performance comparison of passive baseline with different data.* 
    >
    > | Method             |  Acc. (%) | Dodging ASR (%) |         |         |          |          | Impersonation ASR (%) |         |         |         |         |
    > | ------------------ | --------: | --------------: | ------: | ------: | -------: | -------: | --------------------: | ------: | ------: | ------: | :-----: |
    > |                    |           |             MIM |     EoT |   GenAP |    3DAdv |     Adpt |                   MIM |     EoT |   GenAP |   3DAdv |  Adpt   |
    > | *SAC-2D$^\dagger$* |   *86.22* |          *74.5* |  *82.9* |  *81.9* |   *75.5* |   *48.9* |                *45.0* |  *49.0* |  *68.0* |  *61.0* |  *N/A*  |
    > | *PZ-2D$^\dagger$*  |   *88.78* |          *61.1* |  *66.7* |  *85.6* |   *76.7* |     74.0 |                *48.5* |  *51.5* |  *84.8* |  *75.8* | *69.7*  |
    > | SAC$^\dagger$      |     80.55 |            78.8 |    78.6 |    79.6 |     85.8 |     85.0 |                   3.2 |     3.2 |    18.9 |    22.1 |  51.7   |
    > | PZ$^\dagger$       |     85.85 |             6.1 |     6.2 |    14.3 |     20.4 |     69.4 |               **3.1** |     3.2 |    19.1 |    27.4 |  61.0   |
    > | **EAD (ours)**     | **90.45** |         **0.0** | **0.0** | **2.1** | **13.7** | **22.1** |                   4.1 | **3.1** | **5.1** | **7.2** | **8.3** |

3. **Computational Overhead for EAD Defense:** _Training time, memory resources, and wall clock time at both training and inference phases._

    >  We compare our method with the other passive defense baselines. We can tell from the results that our method achieves a better performance with considerable computational overhead in both training and testing. 
    >
    >  *Table 2. Computational overhead comparison of different defense methods in face recognition. We report the training and inference time of defense on a NVIDIA GeForce RTX 3090 Ti and an AMD EPYC 7302 16-Core Processor with the training batch size as 64.* 
    >
    >  | **Method** | **# Params (M)** | **Description**               | **Training Epochs** | **Training Time per batch (s)** | **Inference Time per instance (ms)** |
    >  | ---------- | ---------------- | ----------------------------- | ------------------- | ------------------------------- | ------------------------------------ |
    >  | JPEG       | -                | non-parametric                | -                   | -                               | 9.65                                 |
    >  | LGS        | -                | non-parametric                | -                   | -                               | 26.22                                |
    >  | SAC        | 44.71            | segmenter                     | 50 + 10             | 0.152 / 4.018                   | 26.43                                |
    >  | PZ         | 44.71            | segmenter                     | 50 + 10             | 0.152 / 4.018                   | 11.88                                |
    >  | DOA        | 43.63            | adversarial training          | 100                 | 1.73                            | 8.10                                 |
    >  | EAD (ours) | 57.30            | policy model and fusion model | 50 + 50             | 0.595 / 1.021                   | 38.38 (4 steps)                      |
    >
    >  As for the detailed model training, we train EAD with the configuration in Appendix C.4.  In the offline stage, we train EAD with 2 NVIDIA Tesla A100 for about 4 hours (210 min). Owing to the huge memory consumption of EG3D differential rendering, we resort to train EAD with 8 NVIDIA Tesla A100, and it lasts about 14 hours (867 min). We provide a detailed training curve of EAD in the newly updated appendix.

4. **Computational Overhead for Adaptive Attack:** _Detailed computational cost and feasibility._

    > **Answer:**  In the original version of the paper, the backpropagation through single step requires almost 24GB. owing to the great memory overhead of differential rendering of EG3D. Currently, we utilize the gradient-checkpointing technique to make it possible on a single RTX-3090. The detailed results as well as and newly designed adaptive attacks against single component are provided as follows:
    >
    > We have designed 3 new adaptive attacks to evaluate the robustness of the EAD model: 1) attack the perception model to disrupt the model belief (perception)according to your advice and the work by Sabour et. al.  2) attack the policy model (policy) to make it ensure zero action (i.e. EAD model stay stills) 3) Luckily, we succeed in attacking the whole pipeline along 4-steps trajectory with gradient-checkpointing technique (overall) which hasn't been used previously. 
    >
    > *Table 3. Evaluation of adaptive attacks on the EAD Model. Columns with \emph{USP} represent results obtained by optimizing the patch with an expected gradient over the Uniform Superset Policy (USP). And \emph{perception} and \emph{policy} separately represent adaptive attacks against a single sub-module. And \emph{overall} denotes attacking EAD by following the gradients along the overall (4 step) trajectory with gradient checkpointing.*
    >
    > |             | **Dodging** |                |            |             | **Impersonation** |                |            |             |
    > | :---------: | ----------- | :------------: | :--------: | :---------: | :---------------: | :------------: | :--------: | :---------: |
    > |             | **USP**     | **Perception** | **Policy** | **Overall** |      **USP**      | **Perception** | **Policy** | **Overall** |
    > | **ASR (%)** | **22.11**   |     10.11      |   16.84    |    15.79    |       8.33        |      1.04      |  **9.38**  |    7.29     |
    >
    > The results, as shown in the table, highlight that our original adaptive attack with Uniform Superset Policy (USP) is the most effective in dodging attacks. Though faced with diverse adaptive attacks, our method remains effective. The detailed methodologies of these adaptive attacks are now illustrated in the revised appendix.

5. _Experimental Settings' Sufficiency and Scalability._(*)

> **Answer:** In the training, from the 3D model of 2500 identities, we are able to render a relatively large quantity and diverse 2D face images according to certain protocols (e.g., mixture protocol in the evaluation ...) (~49791 * 16 are used images for training passive baselines and the offline phases, and 49791 * num_epoch images are used to train the online phase)

Your constructive feedback has been instrumental in refining our research. We hope our revised submission now effectively communicates the novel contributions of our proactive defense strategy. We hope that our revisions adequately significantly improve the quality of our manuscript. We remain open to further suggestions and are eager to improve our work to meet the esteemed standards of the conference.

## Reviewer u8yn

Firstly, I want to express my sincerest appreciation for your thoughtful and detailed review of our submission. Your suggestions have been invaluable in enhancing the quality and clarity of our paper.

1. **Details of Adaptive Attack:** _Effectiveness of a surrogate uniform superset policy distribution._

    >  Your query regarding the effectiveness of a surrogate uniform superset policy distribution is pertinent. To empirically validate its effectiveness, we designed three novel adaptive attacks aimed at evaluating the robustness of the EAD model: 1) An attack targeting the perception model to disrupt its belief system, inspired by your suggestion and Sabour et al.'s work; 2) An attack on the policy model to enforce a state of inaction in the EAD model; 3) A successful attack on the entire pipeline using a four-step trajectory with gradient-checkpointing technique, an approach not previously utilized. 
    >
    >  *Table 1. Evaluation of adaptive attacks on the EAD Model. Columns with \emph{USP} represent results obtained by optimizing the patch with an expected gradient over the Uniform Superset Policy (USP). And \emph{perception} and \emph{policy} separately represent adaptive attack against single sub-module. And \emph{overall} denotes attacking EAD by following the gradients for along the overall (4 step) trajectory with gradient checkpointing.*
    >
    >  |             | **Dodging** |                |            |             | **Impersonation** |                |            |             |
    >  | :---------: | ----------- | :------------: | :--------: | :---------: | :---------------: | :------------: | :--------: | :---------: |
    >  |             | **USP**     | **Perception** | **Policy** | **Overall** |      **USP**      | **Perception** | **Policy** | **Overall** |
    >  | **ASR (%)** | **22.11**   |     10.11      |   16.84    |    15.79    |       8.33        |      1.04      |  **9.38**  |    7.29     |
    >
    >  As demonstrated in Table 1, our originally proposed adaptive attack employing Uniform Superset Policy  (USP) proved the most effective in dodging an attack, and only falls slightly behind the attack against the policy module. Though faced with diverse adaptive attacks, our method remains effective. The detailed methodologies of these adaptive attacks are now illustrated in the revised appendix.

2. _Enhancing Passive Defense Models with 3D-Augmented Data._

    >  We apologize for the oversight in not explicitly stating the use of 3D-augmented data in our paper. Indeed, we incorporated images rendered from diverse viewpoints to train the passive baseline. Subsequent training of the baseline exclusively with 2D data led to the expected degradation in performance. The table below provides a detailed comparison of standard accuracy and adversarial attack success rates on Face Recognition (FR) models, highlighting the benefits of 3D-augmented data in enhancing model robustness.
    >
    >  *Table 2. Performance comparison of passive baseline with different data.* 
    >
    >  | Method             |  Acc. (%) | Dodging ASR (%) |         |         |          |          | Impersonation ASR (%) |         |         |         |         |
    >  | ------------------ | --------: | --------------: | ------: | ------: | -------: | -------: | --------------------: | ------: | ------: | ------: | :-----: |
    >  |                    |           |             MIM |     EoT |   GenAP |    3DAdv |     Adpt |                   MIM |     EoT |   GenAP |   3DAdv |  Adpt   |
    >  | *SAC-2D$^\dagger$* |   *86.22* |          *74.5* |  *82.9* |  *81.9* |   *75.5* |   *48.9* |                *45.0* |  *49.0* |  *68.0* |  *61.0* |  *N/A*  |
    >  | *PZ-2D$^\dagger$*  |   *88.78* |          *61.1* |  *66.7* |  *85.6* |   *76.7* |     74.0 |                *48.5* |  *51.5* |  *84.8* |  *75.8* | *69.7*  |
    >  | SAC$^\dagger$      |     80.55 |            78.8 |    78.6 |    79.6 |     85.8 |     85.0 |                   3.2 |     3.2 |    18.9 |    22.1 |  51.7   |
    >  | PZ$^\dagger$       |     85.85 |             6.1 |     6.2 |    14.3 |     20.4 |     69.4 |               **3.1** |     3.2 |    19.1 |    27.4 |  61.0   |
    >  | **EAD (ours)**     | **90.45** |         **0.0** | **0.0** | **2.1** | **13.7** | **22.1** |                   4.1 | **3.1** | **5.1** | **7.2** | **8.3** |

3. Typo in the algorithm box.

    > We are deeply sorry for the typographical errors in the algorithm box, which may have caused confusion. We have diligently corrected these errors in the revised version of the paper. Your keen eye for detail has significantly contributed to improving the accuracy and clarity of our work.

In closing, we appreciate your constructive feedback, which has been instrumental in refining our work. We hope that our revisions adequately address your concerns and significantly improve the quality of our manuscript.

## Reviewer YXUb

First and foremost, I would like to extend my heartfelt gratitude for your thorough and insightful review of our manuscript. Your meticulous attention to detail and constructive feedback are immensely appreciated, and they have significantly contributed to enhancing the quality of our work.

Regarding your queries and suggestions:

1. _Details or examples of actions and states and their physical meanings._

    >  To provide a clearer understanding of the actions and states and their physical meanings within the context of our work, we have enriched the newly modified appendix with detailed examples. These examples will illustrate the practical applications and implications of actions and states in the framework of Embodied Active Defense (EAD), thereby offering a more comprehensive perspective.

2. **Computational Overhead:** _Complexity for training and inference._

    > We have conducted a comparative analysis of our method against other passive defense baselines. The results indicate that our method achieves superior performance, albeit with a considerable computational overhead during both the training and testing phases. The table below presents a comparison of the computational overheads of different defense methods in face recognition, detailing the training and inference time metrics.
    >
    > *Table 1. Computational overhead comparison of different defense methods in face recognition. We report the training and inference time of defense on a NVIDIA GeForce RTX 3090 Ti and an AMD EPYC 7302 16-Core Processor with the training batch size as 64.* 
    >
    > | **Method** | **# Params (M)** | **Description**                    | **Training Epochs** | **Training Time per batch (s)** | **Inference Time per instance (ms)** |
    > | ---------- | ---------------- | ---------------------------------- | ------------------- | ------------------------------- | ------------------------------------ |
    > | JPEG       | -                | non-parametric                     | -                   | -                               | 9.65                                 |
    > | LGS        | -                | non-parametric                     | -                   | -                               | 26.22                                |
    > | SAC        | 44.71            | segmenter                          | 50 + 10             | 0.152 / 4.018                   | 26.43                                |
    > | PZ         | 44.71            | segmenter                          | 50 + 10             | 0.152 / 4.018                   | 11.88                                |
    > | DOA        | 43.63            | adversarial training               | 100                 | 1.73                            | 8.10                                 |
    > | EAD (ours) | 57.30            | policy model and perception  model | 50 + 50             | 0.595 / 1.021                   | 38.38 (4 steps)                      |
    >
    > or detailed model training, EAD was trained using the configuration outlined in Appendix C.4. In the offline stage, EAD training took approximately 4 hours (210 min) on 2 NVIDIA Tesla A100 GPUs. Due to the significant memory requirements of EG3D differential rendering, we employed 8 NVIDIA Tesla A100 GPUs for training, which lasted around 14 hours (867 min). The detailed training curve of EAD is provided in the updated appendix for further insights.

---

## Further Comments

- The paper requires fixing of typos and improvement in clarity.




